Remember When It Matters: Proactive Memory Agent for Long-Horizon Agents

In long-horizon tasks, decision-relevant state is often scattered across an expanding trajectory, while the action agent must surface it and act. As trajectories grow, task requirements, environment facts, prior attempts, diagnoses, and open subgoals can be buried in the context window or pushed beyond it, failing to influence decisions when needed. We call this failure mode "behavioral state decay". We study memory as an active intervention mechanism rather than passive retrieval. A separate memory agent runs alongside an unmodified action agent, updating a structured memory bank from the recent trajectory and deciding whether to inject a memory-grounded reminder or remain silent. The module is plug-and-play with frontier action agents and existing agent harnesses. Across Terminal-Bench 2.0 and $\tau^2$-Bench, it improves pass@1 for both weaker and stronger action agents, with gains of +8.3 pp on Terminal-Bench and +6.8 pp on $\tau^2$-Bench. Ablations show that selective intervention outperforms passive bank exposure, always-on injection, advisor-only guidance, and general retrieval. As an early step toward open-weight memory policies, we train Qwen3.5-27B on SETA using SFT and GRPO, improving validation reward and achieving partial transfer to Terminal-Bench.

==> sections/10_ethics.tex <==
\section*{Ethical Considerations}
We utilize GPT-based models \citep{openai2023gpt4} solely for language polishing
and proofreading.
%
This work studies a memory intervention architecture for long-horizon language
agents using public benchmark environments (Terminal-Bench 2.0, $\tau^2$-Bench,
and SETA) and does not introduce new datasets containing personal or sensitive
information.
%
Our open-weight memory agent use training data written from a frontier-model memory teacher,
so biases or unsafe preferences in the teacher may be propagated to the student;
because the memory agent injects natural-language reminders into the action
loop, such biases can also be amplified at inference time.
%
Practical deployment should therefore include appropriate action validation,
safety constraints, logging, and human oversight.


==> sections/9_limitations.tex <==
\section*{Limitations}

Our memory architecture introduces additional computation. Each memory step
invokes a separate LLM call that processes the recent trajectory window and
the current memory bank, adding token and latency overhead on top of the
action agent. For frontier-model deployments this can roughly double the
inference cost on steps where memory is triggered. Cheaper trigger functions,
shorter trajectory windows, and distillation into smaller memory models are
natural directions for reducing this cost.

Our training results are also preliminary. We train an open-weight memory
agent with SFT and a single-turn GRPO recipe over pivot turns, but have not
yet explored multi-turn RL training in which the memory and action agents are
optimized jointly across full trajectories. Multi-turn RL is our planned
next step: it would replace offline pivot-turn labels with proper
trajectory-level credit assignment, and could yield intervention policies
that adapt to the action agent's behavior rather than imitating a prompted
teacher.

